Petrov-Galerkin Dynamical Low Rank Approximation:SUPG stabilisation of advection-dominated problems

We propose a novel framework of generalised Petrov-Galerkin Dynamical Low Rank Approximations (DLR) in the context of random PDEs. It builds on the standard Dynamical Low Rank Approximations in their Dynamically Orthogonal formulation. It allows to seamlessly build-in many standard and well-studied stabilisation techniques that can be framed as either generalised Galerkin methods, or Petrov-Galerkin methods. The framework is subsequently applied to the case of Streamine Upwind/Petrov Galerkin (SUPG) stabilisation of advection-dominated problems with small stochastic perturbations of the transport field. The norm-stability properties of two time discretisations are analysed. Numerical experiments confirm that the stabilising properties of the SUPG method naturally carry over to the DLR framework.

==> sdraft/SUPG-stochb.tex <==
The stabilisation method proposed in Section~\ref{subsec:stabdlrsche} does not allow to handle the case of a stochastic flow term $\bu(x, \omega)$.
As discussed, such a term cannot simply be put in the standard SUPG formulation and subsequently derive evolution equations for the individual modes. 
We propose the following strategy to handle advection terms admitting a low-rank representation $\bu(x, \omega) = \tilde{b}_0(x) + \sum_{i=1}^K b_i(x) \tilde{\xi}_i(\omega)$, where $\mathbb{E}[\tilde{\xi}(\omega)] = 0$ and $\mathrm{sup}_{\omega \in \Omega} |\tilde{\xi}(\omega)_i| \leq \tilde{K}_i$.   

Denoting $K_i = \tilde{K_i} + \delta$ for some $\delta > 0$, it is possible to rewrite
\begin{align}
	\bu(x,\omega) &= \tilde{b}_0(x) - \sum_{i=1}^K b_i(x) K_i + \sum_{i=1}^K b_i(x) (\tilde{\xi}_i(\omega) + K_i) \nonumber \\
		     &=b_0(x) + \sum_{i=1}^K b_i(x) \xi_i(\omega), \label{eqn:stochb}
\end{align}
where now $\xi(\omega) > \delta$ for $1 \leq i \leq K$.
The strategy is solving the problem in a splitting fashion, firstly solving by stabilising with $\bu = b_0$, then $\bu = b_i(x) \xi_i(\omega)$ for $i=1,\ldots,R$. Indeed, the problem can be rewritten
\[
\partial_t u + \sum_{i=0}^K A_i u = 0,
\]
 where $ (K+1) A_i u = - \varepsilon \Delta u + (K+1) b_i(x) \xi_i (\omega) \cdot \nabla u + cu - f  $ (for notational convenience, $\xi_0 = 1$). 

The framework developed in this paper exactly allows to stabilise the problem a term $\partial_t u + A_0 u = 0$. For the other terms, notice that
\begin{gather}
	\partial_t u + A_i = 0 \nonumber \\
	\iff \partial_t u - \frac{\varepsilon}{K+1} \Delta u + b_i(x) \xi_i(\omega) \cdot \nabla u + \frac{c}{K+1}u  = \frac{f}{K+1}\nonumber \\
	\iff \frac{1}{\xi_i }\partial_t u - \frac{\varepsilon}{\xi_i (K+1) } \Delta u + b_i(x) \cdot \nabla u + \frac{c}{\xi_i (K+1) }u  = \frac{f}{\xi_i (K+1) } \nonumber \\
	\iff \frac{1}{\xi_i }\partial_t u - \frac{\tilde{\varepsilon}}{\xi_i } \Delta u + b_i(x) \cdot \nabla u + \frac{\tilde{c}}{\xi_i }u  = \frac{\tilde{f}}{\xi_i }. 
\end{gather}
The SUPG-stabilised weak form then reads 
\begin{multline}
(\frac{1}{\xi_i}\partial_t u, v) + (\frac{\tilde{\varepsilon}}{\xi_i} \nabla u, \nabla v) + (b_i \cdot \nabla u, v) + (\frac{\tilde{c}}{\xi_i}u, v)  
\\
+ 
\sum_{K \in \Th} \delta_K (\frac{1}{\xi_i}\partial_t u - \frac{\tilde{\varepsilon}}{\xi_i}\Delta u + b_i \cdot \nabla u + \frac{\tilde{c}}{\xi_i}u, b_i \cdot \nabla v)_K
= (\frac{\tilde{f}}{\xi_i}, v) + \sum_{K \in \Th} \delta_K  (\frac{\tilde{f}}{\xi_i}, b_i \cdot \nabla v)_K.
\end{multline}
Collecting the terms with the time derivative and rearranging yields
\begin{equation}
	(\partial_t u, (I + \sum_{K \in \Th} \delta_K \; \chi_K \; b_i(x) \cdot \nabla) \frac{1}{\xi_i} v) =
	(\partial_t u, \Hcal_1 \otimes \Hcal_2 v),
\end{equation}
where $\Hcal_2$ induces a scalar product. The framework developed previously can be used to solve this sub-problem. The time-marching scheme then reads as follows:

\setcounter{algorithm}{1}
\begin{algorithm}
\caption{Splitting algorithm}\label{alg:cap}
\begin{algorithmic}[1]
\Require $\uhr[n,(0)]$
%\Ensure $y = x^n$
\For{$i = 0, \dots, K$}
\State Reparametrise $\uhr[n,(i)] = U_0 Y_0 + \sum_{i=1}^R U_i Y_i$ s.t. $\mathbb{E}[\frac{1}{\xi_i}Y_j Y_k] = \delta_{jk}$, $\mathbb{E}[\frac{1}{\xi_i} Y_k] = 0$ for $1 \leq k \leq R$, $0 \leq j \leq R$.
%$\mathbb{E}[\frac{1}{\xi} \mathbbm{1}] = 1$
\State Solve the DLR problem to $\partial_t u + A_i u = 0$ on $[t_n, t_{n+1}]$ with stabilisation
\State $\uhr[n,(i+1)] \gets \uhr[n+1,(i)]$
\EndFor
\State $\uhr[n+1] = \uhr[n+1,(K)]$
\end{algorithmic}
\end{algorithm}

%\todo{Need to discuss what happens to the mean part? }


==> sdraft/ee-stab.tex <==
The explicit-Euler discretisation variational formulation is given by
\begin{multline} \label{eqn:varf-ee}
	\frac{1}{\dt}(U^n_h - U^{n-1}_h, v_h) + \varepsilon(\nabla U^{n-1}_h, \nabla v_h) + (\bu  \cdot \nabla  U^{n-1}_h, v_h) + (c U^{n-1}_h, v_h) 
	\\ + \sum_{K \in \mathcal{T}_{\!h}} \frac{\delta_K}{\dt}(U^{n}_h - U^{n-1}_h, \bu \cdot \nabla v_h)_K + \delta_K (-  \varepsilon \Delta U^{n-1}_h + \bu \cdot \nabla U^{n-1}_h + cU^{n-1}_h, \bu  \cdot \nabla v_h)_K \\ 
	= (f,v_h) + \sum_{K \in \mathcal{T}_{\!h}} \delta_K (f, \bu \cdot \nabla v_h)_{K} \quad \forall v_h \in V_{h,r}.
\end{multline}



\begin{theorem} \label{th:bound1}
	Assuming $\delta_K$ satisfies~\eqref{eqn:deltaK-coerc} and 
	\begin{equation}
		\delta_K \leq \min\left\{ \dt, \frac{1}{320} \max\left\{ \frac{h^4}{\varepsilon^2 C_I^2}, \frac{h^2}{C_I^2 \|\bu\|^2_{L^{\infty}(K)}}, \frac{1}{\|c\|_{L^{\infty}(K)}}, 1  \right\}  \right\}
	\end{equation}
	and under the condition
	\begin{equation}
		\dt \leq \min \left\{ \frac{\theta h^2}{2 \varepsilon C_I^2}, \frac{\eta h^2}{\|c\|_{L^{\infty}(\Omega)}}, \frac{\eta}{\|c\|_{L^{\infty}(\Omega)}}, 8 \theta\right\}
	\end{equation} 
	for some $0 < \theta < \frac{1}{2}$ and $\eta > 0$, the following holds:
	\begin{multline}	
		\| U^n_h \|^2 + \dt (\frac{1}{2} - \theta) \sum_{n=1}^N \|U^n_h\|^2_{\mathrm{SUPG}} \leq \left( \|U^0_h\|^2 + \dt \sum_{n=0}^{N-1} C(f^k) \right) \exp(\eta T), 
	\end{multline}
	where 
	\[
		C(f^n) \coloneq \frac{1}{\mu_0} + \frac{5}{\theta} \sum_{K \in \mathcal{T}_{\!h}} \delta_K \| f^n  \|^2_K
	\]
\end{theorem}
\begin{proof}
	We consider the variational formulation and use the linearity to obtain
\begin{multline*} 
	\frac{1}{\dt}(U^n_h - U^{n-1}_h, v_h) + a_{\mathrm{SUPG}}(U^{n-1}_h  - U^n_h, v_h)+ a_{\mathrm{SUPG}}(U^n_h, v_h) \\
	 + \sum_{K \in \mathcal{T}_{\!h}} \frac{\delta_K}{\dt}(U^{n}_h - U^{n-1}_h, \bu \cdot \nabla v_h)_K = (f,v_h) + \sum_{K \in \mathcal{T}_{\!h}} \delta_K (f, \bu \cdot \nabla v_h)_{K} \quad \forall v_h \in V_{h,r}.
\end{multline*}
We test against $U^{n}_h$ and bound the terms. Recall that $a_{\mathrm{SUPG}}$ is coercive, i.e. we have: 
\[
	a_{\mathrm{SUPG}}(U^n_h,U^n_h) \geq \frac{1}{2}\|U^n_h\|^2_{\mathrm{SUPG}}.
\]
	Furthermore, 
\begin{multline*}
	a_{\mathrm{SUPG}}(U^{n-1}_h - U^{n}_h, v_h) =
	\\
	\varepsilon(\nabla (U^{n-1}_h - U^n_h), \nabla v_h) + (\bu  \cdot \nabla  (U^{n-1}_h- U^n_h), v_h) + (c (U^{n-1}_h - U^n_h), v_h) \\ + \sum_{K \in \mathcal{T}_{\!h}} \delta_K (-  \varepsilon \Delta (U^{n-1}_h - U^{n}_h) + \bu \cdot \nabla (U^{n-1}_h - U^n_{h}) + c(U^{n-1}_h - U^n_h), \bu  \cdot \nabla v_h)_K 
\end{multline*}
We then bound the first $3$ terms as 
	\begin{align*}
		|\varepsilon(\nabla (U^{n-1}_h - U^n_h), \nabla U^{n}_h)| 
		&\geq - \varepsilon \frac{C_I}{h} \| U^{n-1}_h - U^n_h \| \| \nabla U^n_h\|
		\\
		&\geq - \varepsilon \frac{C_I^2}{\theta h^2} \| U^{n-1}_h - U^n_h \|^2 - \theta\varepsilon \| \nabla U^n_h\|^2, 
		\\
		|(\bu  \cdot \nabla  (U^{n-1}_h - U^{n}_h), U^{n}_h)| &\geq - \| \bu \|_{L^{\infty}(\Omega)}\frac{C_I}{h}\|U^{n}_h - U^{n-1}_h\| \|U^n_h\|
		\\
&\geq - \frac{\| \bu \|^2_{L^{\infty}(\Omega)}  C_I^2}{2\eta h^2}\|U^{n}_h - U^{n-1}_h\|^2 - \frac{\eta}{2}\|U^n_h\|^2 \\
		|(c U^{n-1}_h - U^n_h,  U^{n}_h)| &\geq - \|c\|_{L^{\infty}(\Omega)} \|U^{n}_h - U^{n-1}_h\| \|U^{n-1}_h\|, 
		\\
		&\geq - \frac{\|c\|_{L^{\infty}(\Omega)}}{2\eta} \|U^{n}_h - U^{n-1}_h\|^2 - \frac{\eta}{2} \|U^{n-1}_h\|^2. 
	\end{align*}
Proceeding in a similar fashion for the $3$ latter terms, we have
\begin{align*}
		|(\varepsilon(\Delta (U^{n-1}_h - U^n_h), \bu \nabla U^{n}_h)_K| 
		&\geq -\frac{5\varepsilon^2 C_I^4}{\theta h^4} \| U^{n-1}_h - U^n_h \|^2_K - \frac{\theta}{5}\| \bu \nabla U^n_h\|^2_K, 
		\\
		|(\bu  \cdot \nabla  (U^{n-1}_h - U^{n}_h), \bu \cdot \nabla U^{n}_h)_K| 
		%&\geq - \| \bu \|_{L^{\infty}(K)}\frac{C_I}{h}\|U^{n}_h - U^{n-1}_h\| \|U^n_h\|
&\geq - \frac{5 \| \bu \|^2_{L^{\infty}(K)}  C_I^2}{\theta h^2}\|U^{n}_h - U^{n-1}_h\|^2_K - \frac{\theta}{5}\|\bu \cdot \nabla U^n_h\|^2_K \\
		|(c U^{n-1}_h - U^n_h, \bu \cdot \nabla  U^{n}_h)_K| 
		%&\geq - \|c\|_{L^{\infty}(K)} \|U^{n}_h - U^{n-1}_h\| \|U^{n-1}_h\|, 
		&\geq - \frac{5\|c\|_{L^{\infty}(K)}}{\theta} \|U^{n}_h - U^{n-1}_h\|^2_K - \frac{\theta}{5} \|\bu \cdot \nabla U^{n}_h\|^2. 
\end{align*}

%	\begin{multline*}
%		(\bu  \cdot \nabla  U^{n-1}_h, U^{n}_h) =  + (\bu  \cdot \nabla  U^{n}_h, U^{n}_h)
%		\\
%							\geq -\frac{1}{2}\int_{\Omega} \mathrm{div}\;\bu (U^{n}_h)^2  + \frac{1}{2}\int_{ \partial \Omega} \bu\cdot\mathbf{n} (U^{n}_h)^2 		\\
%		= -\frac{1}{2}\int_{\Omega} \mathrm{div}\;\bu (U^{n}_h)^2 - \| \bu \|_{L^{\infty}}\frac{C_I}{h}\|U^{n}_h - U^{n-1}_h\| \|U^n_h\|
%		%(c U^{n-1}_h,  U^{n}_h) &= 
%	\end{multline*}
We bound the remaining terms as follows:
\begin{align*}
	(f^n,U^n_h) &\leq \frac{1}{\theta}\|\mu^{-1/2}f^n\|^2 + \theta\| \mu^{1/2} U^n_h  \|^2 \leq \frac{1}{\mu_0 \theta}\|f^n\|^2 + \theta\| \mu^{1/2} U^n_h  \|^2\\
         (f^n, \bu \cdot \nabla U^n_h)_{K} &\leq \frac{5}{\theta}\| f^n \|^2_{K} +  \frac{\theta}{5}\| \bu \cdot \nabla  U^n_h \|^2_K  \\
	 (U^n_h - U^{n-1}_h, \bu \cdot \nabla U^n_h )_K &\leq \frac{5}{\theta }\|U^n_h - U^{n-1}_h\|^2_K + \frac{\theta }{5 } \|\bu \cdot \nabla U^n_h\|^2_K
\end{align*}
Combining these results, we have that
\begin{multline*}
	a_{\mathrm{SUPG}}(U^{n-1}_h - U^n_h,U^n_h) +  \sum_{K \in \mathcal{T}_{\!h}} \frac{\delta_K}{\dt}(U^{n}_h - U^{n-1}_h, \bu \cdot \nabla U^n_h)_K 
	- (f,U^n_h) 
	\\ - \sum_{K \in \mathcal{T}_{\!h}} \delta_K (f, \bu \cdot \nabla U^n_h)_{K} \geq - \left( \frac{\varepsilon C_I^2}{\theta h^2} +  \frac{\| \bu \|^2_{L^{\infty}(\Omega)}  C_I^2}{2\eta h^2} + \frac{\|c\|_{L^{\infty}(\Omega)}}{2\eta}  \right) \|U^n_h - U^{n-1}_h\|^2  
	\\ - \eta \|U^n_h\|^2 	- \sum_{K \in \mathcal{T}_{\!h}} \delta_K \left( \frac{5\varepsilon^2 C_I^4}{\theta h^4} + \frac{5 \| \bu \|^2_{L^{\infty}(K)}  C_I^2}{\theta h^2} + \frac{5\|c\|_{L^{\infty}(K)}}{\theta} + \frac{5}{\theta}  \right) \|U^n_h - U^{n-1}_h\|^2_K 
	\\ - \theta \sum_{K \in \mathcal{T}_{\!h}} \delta_K \| \bu \cdot U^n_h\|^2_K - \theta \varepsilon \| \nabla U^n_h  \|^2 -  \theta\| \mu^{1/2} U^n_h  \|^2  - \frac{1}{\mu_0 \theta}\|f^n\|^2 - \frac{5}{\theta} \sum_{K \in \mathcal{T}_{\!h}} \delta_K   \| f^n \|^2_{K} 
	\\ \geq -\theta \|U^n_h\|^2_{\mathrm{SUPG}} - \eta \| U^n_h \|^2 - \left( \frac{\varepsilon C_I^2}{\theta h^2} +  \frac{\| \bu \|^2_{L^{\infty}(\Omega)}  C_I^2}{2\eta h^2} + \frac{\|c\|_{L^{\infty}(\Omega)}}{2\eta} + \frac{1}{16\theta}  \right) \|U^n_h - U^{n-1}_h\|^2
	\\ - \frac{1}{\mu_0 \theta}\|f^n\|^2 - \frac{5}{\theta} \sum_{K \in \mathcal{T}_{\!h}} \delta_K   \| f^n \|^2_{K}. 
\end{multline*}
Finally, using the fact that 
\[
	(U^n_h - U^{n-1}_h, U^n_h) = \frac{1}{2}\left( \|U^n_h\|^2 - \|U^{n-1}_h  \|^2 + \|U^n_h - U^{n-1}_h \|^2  \right), 
\]
by testing against $U^n_h$ we obtain
\begin{multline*}
	\frac{1}{2\dt}(\|U^n_h\|^2 -  \|U^{n-1}_h\|^2) + \left(\frac{1}{2\dt} - \frac{\varepsilon C_I^2}{\theta h^2} -  \frac{\| \bu \|^2_{L^{\infty}(\Omega)}  C_I^2}{2\eta h^2} -  \frac{\|c\|_{L^{\infty}(\Omega)}}{2\eta} - \frac{1}{16 \theta}  \right)  \|U^n_h - U^{n-1}_h\|^2) 
	\\
	+ \left( \frac{1}{2} - \theta \right) \|U^n_h\|^2_{\mathrm{SUPG}}  
	\leq \eta \|U^{n-1}_h\|^2 + \frac{1}{\mu_0} \|f^n\|^2 + \frac{5}{\theta} \sum_{K \in \mathcal{T}_{\!h}} \delta_K \|f^n\|^2_K
\end{multline*}

\end{proof}

Another way to obtain a similar result is given by testing against $U^{n-1}_h$, from which we obtain
\begin{multline*}
	\frac{1}{2\dt} (\|U^n_h\|^2 +  \|U^{n-1}_h\|^2 -  \|U^n_h - U^{n-1}_h\|^2) + \frac{1}{2}\|U^{n-1}\|_{\mathrm{SUPG}}^2  \\ \leq \frac{1}{4\dt}\|U^n - U^{n-1}\|^2 +  \left( \frac{2}{\mu_0} + \dt \right)\|f_n\|^2 
\end{multline*}
where we have used the same method as in Theorem~\ref{th:bound1} to bound
\[
\sum_{K \in \mathcal{T}_h} \frac{\delta_K}{\dt} (U^n_h - U^n_h, \mathbf{b} \cdot \nabla U^{n-1}_h) \leq \frac{1}{4\dt} \|U^n_h - U^{n-1}_h\|^2 + \sum_{K} \delta_K \| \bu \cdot \nabla U^{n-1}_h\|^2_K 
\]
which works under the assumption $4\delta_K \leq \dt$ (the latter term is absorbed into the$a_{\mathrm{SUPG}}$ term).
Therefore, we only need to control the term $\frac{3}{4} \|U^n_h - U^{n-1}_h\|^2$ in order to get a bound.  
Testing against $U^n_h - U^{n-1}_h$, we obtain a bound of the form
\begin{equation}
	\frac{1}{\dt}\|U^n_h - U^{n-1}_h\| \leq C(h, \varepsilon, \bu, c) \|U^{n-1}_h\| + \|f_n\| + \sum_K \delta_K \|f_n\|_K,
\end{equation}
which we can then use to bound the terms and obtain a Gronwall-like bound under some (likely) parabolic/hyperbolic-type CFL condition (the hyperbolic constraints may dominate). 

TODO: write down full proof...




==> sdraft/norm-stab.tex <==
We consider the advection-diffusion problem 
\begin{equation}
	\dot{u} - \varepsilon(\omega) \Delta u+  
	\bu(x) \cdot \nabla u = 0,
\end{equation}
%furthermore assuming that~\ref{eqn:divb0},~\ref{eqn:muzero} and~\ref{eqn:varepscoer} hold. Finally, we use $\mathbb{P}^C_1(\Th)$ elements, implying that the residual term $- \varepsilon \Delta v_{|K} = 0$ for any $v \in V_h \otimes \Lthm$. \todo{Not happy with ordering of hypotheses} We then have:
\begin{theorem}
	Assuming~\ref{eqn:bdet}-~\ref{eqn:muzero}, and under the condition
\begin{equation} \label{eqn:norm-stab-cfl1}
	\delta_K \leq 2 \dt,
\end{equation}
the iterates of the DLR solution $\{\uhr[k]\}_{k=0}^{N}$ verify:
\begin{equation}
	\| \uhr[N] \|^2_{X,\Lthm} + 2 \dt \epsilon   \sum_{n = 1}^{N} \|\nabla \uhr[n+1] \|^2_{X,\Lthm} \leq \| \uhr[0] \|^2_{X,\Lthm}.  
\end{equation}
\end{theorem}
\begin{proof}
	We first detail a few bounds, and then expand on how those can be used to obtain the different cases. The main ``challenge'' may be suitably bounding with the term $\delta_K \dt{-1}(\uhr[n+1] - \uhr[n], \bu \cdot \nabla \uhr[n+1])_{K,\Lthm}$ -- to this end, we use the same approach as in~\cite{jovo11}, which is where condition~\eqref{eqn:dK-dt-bound}

	Testing against $\uhr[n+1] \in \mathcal{T}_{\tilde{U}^{n+1} {Y^n}^{\top}} \mathcal{M}_{\!R}$ and using the fact that $2(u-v,u) = \|u\|^2 - \|v\|^2 + \|u - v\|^2$, the first term becomes 
	\[
		\frac{1}{2\dt}(\|\uhr[n+1] \|_{X,\Lthm}^2 -  \| \uhr[n] \|_{X,\Lthm}^2 +  \| \uhr[n+1]- \uhr[n] \|_{X,\Lthm}^2). 
	\]
	The second term verifies $(\varepsilon \nabla \uhr[n+1], \nabla \uhr[n+1]) \geq \hat{\varepsilon}\| \nabla \uhr[n+1] \|^2_{X,\Lthm}$
	by~\ref{eqn:varepscoer}. 

	%The third term is obtained by noticing that $2(v, \bu \cdot v) = - \int \mathrm{div} \,\bu \cdot v^2$ by~\ref{eqn:muzero} for any $v \in L^2_{\hat{\mu}}(\hat{\Omega}, H^1_0)$ (since here $c(x,\omega) = 0$, consequently $(\uhr[n+1], \bu \cdot \nabla \uhr[n+1]) \geq 0$. 
	%The last term can easily be rewritten
	%\[
%		\sum_{K \in \Th} \delta_K  (\bu \cdot \nabla  \uhr[n+1], \bu \cdot \nabla \uhr[n+1])_{K,\Lthm} =   \sum_{K \in \mathcal{T}_{\! \!h}} \delta_K \| \bu \cdot \nabla \uhr[n+1] \|^2_{K,\Lthm}. 
	%\]
	Finally, for the second-to-last term, using Cauchy-Schwarz and the $\epsilon$-Young inequality gives
	\begin{multline}
	\left| 
		\sum_{K \in \mathcal{T}_{\!\!h}} \frac{\delta_K}{\dt} (\uhr[n+1] - \uhr[n], \bu \cdot \nabla \uhr[n+1])_{K,\Lthm}
	\right|
	\\ \leq 
	\sum_{K \in \mathcal{T}_{\!\!h}} \frac{\delta_K}{\dt} \left(\frac{\| \uhr[n+1] - \uhr[n] \|^2_{K,\Lthm}}{2 \cdot 2 \dt} + \frac{ 2\dt \| \bu \cdot \nabla \uhr[n+1]\|_{K,\Lthm}^2}{2} \right) \\
	\leq \sum_{K \in \mathcal{T}_{\!\!h}} \frac{1}{2\dt} \| \uhr[n+1] - \uhr[n] \|^2_{K,\Lthm} +  \delta_K \| \bu \cdot \nabla \uhr[n+1]\|_{K,\Lthm}^2
	\\
	\leq \frac{1}{2\dt} \| \uhr[n+1] - \uhr[n] \|^2_{X,\Lthm} + \sum_{K \in \mathcal{T}_{\!\!h}}  \delta_K \| \bu \cdot \nabla \uhr[n+1]\|_{K,\Lthm}^2, 
	\end{multline}
	where in the third line is obtained using~\eqref{eqn:norm-stab-cfl1}.
	Combining the above relations, 
	\begin{multline}
		\frac{1}{2\dt}(\|\uhr[n+1] \|_{X,\Lthm}^2 -  \| \uhr[n] \|_{X,\Lthm}^2 +  \| \uhr[n+1]- \uhr[n] \|_{X,\Lthm}^2) + \epsilon \| \nabla \uhr[n+1] \|^2_{X,\Lthm} +  \sum_{K \in \mathcal{T}_{\! \!h}} \delta_K \| \bu \cdot \nabla \uhr[n+1] \|^2_{K,\Lthm} \\
	\leq \frac{1}{\dt}(\uhr[n+1] - \uhr[n], \uhr[n+1])_{X,\Lthm} 
	 + (\varepsilon \nabla \uhr[n+1], \nabla \uhr[n+1])_{X,\Lthm} 
	 + (\bu \cdot \nabla  \uhr[n+1], \uhr[n+1])_{X,\Lthm} 
	 \\
	 + \sum_{K \in \Th} \delta_K (\bu \cdot \nabla \uhr[n+1], \bu \cdot \nabla \uhr[n+1])_{K,\Lthm}
	  = - \sum_{K \in \mathcal{T}_{\!h}} \frac{\delta_K}{\dt}(\uhr[n+1] - \uhr[n], \bu \cdot \nabla \uhr[n+1])_{K,\Lthm}
	 \\ 
	 \leq \left| \sum_{K \in \mathcal{T}_{\!h}} \frac{\delta_K}{\dt}(\uhr[n+1] - \uhr[n], \bu \cdot \nabla \uhr[n+1])_{K,\Lthm} 
  \right| 
  \\
  	\leq \frac{1}{2\dt} \| \uhr[n+1] - \uhr[n] \|^2_{X,\Lthm} + \sum_{K \in \mathcal{T}_{\!\!h}}  \delta_K \| \bu \cdot \nabla \uhr[n+1]\|_{K,\Lthm}^2.
	\end{multline}
	Cancelling a few terms, and multiplying by $2\dt$ yields
	\[
	\|\uhr[n+1] \|_{X,\Lthm}^2 -  \| \uhr[n] \|_{X,\Lthm}^2 + 2 \dt \epsilon \| \nabla \uhr[n+1]  \|^2_{X,\Lthm} \leq 0.  
	\]
	The result is obtained by summing for $j = 0, \ldots, N-1$. 
\end{proof}
\todo{Aim of this was to show the practical simplicity of using the variational formulation -- am I achieving this here?}
%The third step in that proof consists in bounding $(\uhr[n+1], \bu \cdot \uhr[n+1]) \geq 0$ -- stronger results would be possible if considering advection-diffusion-reaction equations, and using the standart assumption $c - \frac{1}{2} \mathrm{div} \bu \geq \mu_0 > 0$ (a little more in the spirit of Volker/Novo article). 
%Note that one could relatively easily add a source term on the right-hand-side, which may then be absorbed by $\epsilon \| \nabla \uhr[n+1] \|_{H,\Lthm}$ with $\varepsilon$-Young, at the cost of having a large constant on the rhs. 
%Treating the case of stochastic diffusion and transport through mean-stabilisation should also be possible, combining the approaches of the proofs above.  
%
%The following theorems and proofs follow the same structure; we absorb the potentially negative parts by using Cauchy-Schwarz and $\epsilon$-Young, using the available positive quantities. 
%
%\begin{theorem}
%Under the condition 
%\begin{equation} \label{eqn:norm-stab-cfl2}
%	\delta_K \leq C
%\end{equation}
%we have that
%\begin{equation}
%	%\| \uhr[N] \|^2_{H,\Lthm} + 2 \dt \epsilon   \sum_{n = 1}^{N} \|\nabla \uhr[n+1] \|^2_{H,\Lthm} \leq \| \uhr[0] \|^2_{H,\Lthm}.  
%	a \leq b
%\end{equation}
%
%\end{theorem}
%\begin{proof}
%	Starting from~\eqref{eqn:varf-stochdiff-si}, we test against $\uhr[n+1]$. 
%	%The quantity that must be ensured to be positive is then
%	We note that 
%	\begin{multline}
%		|(\varepsilon^{\star} \nabla \uhr[n] \mp \nabla \uhr[n+1], \nabla \uhr[n+1])| \leq  C_{\mathrm{stoch}} (\| \nabla (\uhr[n] - \uhr[n+1]) \|_{H,\Lthm} \|\nabla \uhr[n+1]\|_{H,\Lthm} + \|\nabla \uhr[n+1]\|^2_{H,\Lthm}) \\
%		\leq \frac{C_{\mathrm{stoch}} C_I^2}{2 h^2} \| \uhr[n+1] - \uhr[n] \|^2_{H,\Lthm} + \frac{3 C_{\mathrm{stoch}}}{2} \| \nabla \uhr[n+1]  \|_{H,\Lthm}^2
%	\end{multline}
%	Furthermore, 
%	\begin{multline}
%	\left| 
%		\sum_{K \in \mathcal{T}_{\!\!h}} \frac{\delta_K}{\dt} (\uhr[n+1] - \uhr[n], \bu \cdot \nabla \uhr[n+1])_{K,\Lthm}
%	\right|
%	\\ 
%	\leq \sum_{K \in \mathcal{T}_{\!\!h}} \frac{\delta_K}{2\dt^2} \| \uhr[n+1] - \uhr[n] \|^2_{K,\Lthm} +  \delta_K \| \bu \cdot \nabla \uhr[n+1]\|_{K,\Lthm}^2
%	\end{multline}
%	\end{proof}

Finally, classical results from the literature can be seamlessly adapted to our setting: 

\begin{theorem}
	(Adapted from \cite[Theorem~3.1]{jovo11}) For a general advection-diffusion-operator such that the hypotheses of Lemma~\ref{lem:coerasupg} hold, and additionally for
	\begin{equation} \label{eqn:deltaK-cond2}
		\delta_K \leq \frac{\dt}{4},
	\end{equation}
	the iterates of the DLR solution $\{\uhr[k]\}_{k=0}^N$ satisfy
	\begin{equation}
		\|\uhr[N]\|^2_{X,\Lthm} + \frac{\dt}{2} \sum_{j=1}^N \|\uhr[n]\|^2_{\mathrm{SUPG}} \leq \|\uhr[0]\|^2_{X,\Lthm} + 2 \left( \frac{2}{\mu_0} + \dt \right) \sum_{j=1}^N \|f\|^2_{X,\Lthm}.
	\end{equation}
\end{theorem}
\begin{proof}
	See~\cite{jovo11}. The proof follows exactly the same steps, as it relies only on testing against $\uhr[n+1]$ and using the hypotheses from Lemma~\ref{lem:coerasupg}. 
\end{proof}

%\todo{check one last time that everything works exactly as claimed}


==> sdraft/numexp1.tex <==
We solve the classical ``rotating'' problem, adapted from~\cite{jovo11, josc08} to the stochastic setting. In the determinstic setting, three ``shapes'' are advected on the domain $D = (0,1)^2$ by a counter-clockwise rotation field with unitary angular velocity centered in $(0.5, 0.5)$; furthermore, as the diffusion is small and there is no reaction term, after $t = 2\pi$ seconds, one expects to recover (almost) the initial condition. 

To adapt this example to our stochastic dynamical low-rank setting, we consider the following coefficients for~\eqref{eqn:adv-diff-reac}, 
\begin{align*}
	\varepsilon(\mathbf{y}) = 10^{y_1 - 16} && \bu(\mathbf{x}) = (0.5 - x_2, x_1 - 0.5)^{\top} && c = 0, 
\end{align*}
where $\mathbf{y} \in \Omega \coloneq [-1, 1]^3 $ is the parameter space, with measure $\displaystyle \mu(\mathrm{d}\mathbf{y}) = \frac{1}{8} \bigotimes_{i=1}^3 \lambda( \mathrm{d} y_i)$, where $\lambda$ is the Lebesgue measure.  
%The stochastic space is discretised, the true solution $u \in L^2_{\hat{\mu}}(\hat{\Omega}, V)$ and will approximate it by the numerical solution in $V_h \otimes \Lthm$. 

%The dynamics at hand are therefore counter-clockwise rotation around $(0.5, 0.5)$ with some small stochastic diffusion. 

The ``shapes'' to be rotated are given by functions $U_0, U_1, U_2$, weighted by stochastic coefficients -- this expansion yields the initial condition. 
Let $r(x_1,x_2) = \sqrt{(x_1 - a)^2 + (x_2 - b)^2}/r_0$, where $r_0 = 0.15$. We then construct
\begin{equation}
	U_0(\mathbf{x}) = 
	\begin{cases}
		1 & \text{ if } r(x,y) \leq 1, \text{ and } |x_1 - a| \geq 0.025, x_2 \geq 0.85
		\\
		0 & \text{ else }
	\end{cases}, 
	\qquad 
	Y_0(\omega) = 1,  
\end{equation}
having used $(a,b) = (0.5, 0.75)$. This corresponds to a slotted cylinder. Next,  
\begin{equation}
	U_1(\mathbf{x}) = \frac{1}{4}(1 + \cos(\pi \min\{r(x_1,x_2), 1\})), \qquad \tilde{Y}_1(\mathbf{y}) = 2 y_1\cos(y_2)
\end{equation}
having set $(x_1, x_2) = (0.25, 0.5)$. This corresponds to a hump. Finally,
\begin{equation}
	U_2(\mathbf{x}) = 1 - \min\{ r(x_1,x_2), 1\}, \qquad \tilde{Y}_2(\mathbf{y}) = 30 y_1 (y_3)^3
\end{equation}
represents a cone, centered at $(a,b) = (0.5, 0.25)$. 

If the problem were a pure advection problem (hyperbolic), the true solution would be of rank $3$ (sum of a deterministic and two random zero-mean functions). The present problem is a singular perturbation of pure advection, and, as it displays a similar solution profile as its hyperbolic counterpart, we set $R=2$. 


For the physical space, we used a uniform triangular mesh $\mathcal{T}_{h}$ of $128 \times 128$ and considered the $\mathbb{P}_1^C(\mathcal{T}_h)$-finite element space, yielding $N_h = 16641$ degrees of freedom. 
The stochastic space was discretised using $N_C = 7000$ independent and uniformly distributed samples from $\Omega$, yielding $\hat{\Omega} = \{{\omega}^{i}\}_{i=1}^{N_C}$. 

To ensure $U_0$ represents the mean of the random field at the discretised level, we subtract the sample mean of each stochastic mode, stack them in a matrix $[\tilde{Y}^{\star}_1, \tilde{Y}^{\star}_2]$, perform a weighted QR-factorisation to obtain a set of $\Lthm$-orthonormal modes, hereafter $Y_1$ and $Y_2$. The initial condition is then given by $u_0(x, \omega) = U_0(x) + \sum_{i=1}^R U_i(x) Y_i(\omega)$. Below, we show one realisation of this function: 
\begin{figure}[h]
\includegraphics[height=9cm]{vn-IC-real-3-3d}
\centering
\caption{A realisation of the initial condition.}
\end{figure}

We chose a time step $\dt = 2\pi / 70000 \approx 10^{-4}$. On the basis of the discussion in~\cite{jovo11}, we set the SUPG parameter to $\delta_K = \nicefrac{h_K}{4}$. We used the semi-implicit time-stepping scheme.  

%In this case, the optimal variance for each mode would be (almost) constant, given respectively by the height of each volume in the initial condition. The results are displayed in Figure~\ref{fig:numexp1-vars}. As can be seen, the slotted cylinder ($U_0$) clearly benefits from using the SUPG formulation; this is unsurprising, as it is the volume presenting the steepest gradients. In the present case, the oscillations born in numerical solution $U_0$ do not ``contaminate'' the other modes, since, as can be seen in the equation~\eqref{eqn:detmodes-adr-si}, the modes only interact through the stochastic diffusion, which is small.   
%
%\begin{figure}[h]
%\includegraphics[width=9cm]{vars-comparison}
%\centering
%\caption{Variances of the indiviual modes. 
%%Corresponding modes are paired through colour. Full lines represent modes obtained through Galerkin method, dotted lines represent modes obtained through SUPG stabilisation.
%}
%\label{fig:numexp1-vars}
%\end{figure}
%
%\begin{figure}[h]
%\includegraphics[width=9cm]{tv-comparison}
%\centering
%\caption{Total variation of the indiviual modes. 
%%Corresponding modes are paired through colour. Full lines represent modes obtained through Galerkin method, dotted lines represent modes obtained through SUPG stabilisation.
%}
%\label{fig:numexp1-tv}
%\end{figure}
%


%Another metric that can be used to compare the two solutions is given by the \textit{total variation} norm, given by

In Figure~\ref{fig:real-dlr-vs-gal}, we display side-by-side one realisation at time $t = 2\pi$ of the numerical solution obtained via the standard DLR method and via the SUPG-stabilised DLR method. As can be observed, we recover a behaviour consistent with what has been discussed in~\cite{jovo11}: the SUPG method considerably damps the oscillations, although it doesn't cancel them entirely.

\begin{figure}[h]
\includegraphics[width=15cm]{vn-real-3-3d}
\centering
\caption{A realisation of the numerical DLR solution obtained through standard Galerkin (left) and through the SUPG-stabilised method (right).} 
%The same color scheme is applied to both plots.}
\label{fig:real-dlr-vs-gal}
\end{figure}

%TODO: should add a table... with realisations!


==> sdraft/numexp2.tex <==
We now consider the case of stochastic advection. This case does not fall into the framework described up to now, as with a stochastic $\bu$, it is not possible to write the operator $\Hcal$ in a separable form. To this end, we propose to stabilise the DLR equations with the mean of the advection field $\bar{\bu}(x)$ -- this approach is only expected to work in the presence of moderate stochasticity. 


We consider the same set-up as before, this time with a constant diffusion $\varepsilon = 10^{-15}$,
\begin{equation*}
	\bu(\mathbf{x}, \omega) = 
	\begin{pmatrix}
		0.5 - y \\
		x - 0.5
	\end{pmatrix} 
	+ \mu \xi_1(\omega)
	\begin{pmatrix}
		y^2 x \\
		-x^2 y
	\end{pmatrix} = \bar{\bu}(\mathbf{x}) + \bu^{\star}(\mathbf{x}, \omega),
\end{equation*}
and again $c = f = 0$. Here, $\xi_1(\omega^i) = \omega^i_3 $. We furthermore set $\mu = 0.1$.  

%For completeness, we write down the equations we use (again, using the semi-implicit integrator):
%%\textit{1. Mean: find $\bar{u}^{n+1} \in V_h$ s.t.}
%\begin{multline} \label{eqn:numexp2-mean}
%	\lrX{\frac{\bar{u}^{n+1} - \bar{u}^n}{\triangle t},v_h} +  
%	\lrX{\varepsilon \nabla \bar{u}^{n+1}, \nabla v_h} 
%	+\lrX{\bar{\bu} \cdot \nabla \bar{u}^{n+1}, v_h} 
%	+\lrX{ \mathbb{E}[{\bu}^{\star} \cdot \nabla u^{n}], v_h} 
%	\\ 
%	+ \sum_{K \in \Th} \frac{\delta_K}{\dt}\langle\bar{u}^{n+1} - \bar{u}^n, \bar{\bu} \cdot \nabla v_h\rangle_K 
%	+ \langle  \bar{\bu} \cdot \nabla \bar{u}^{n+1}  + \mathbb{E}[ \bu^{\star} \cdot \nabla \uhr[n] ], \bar{\bu} \cdot \nabla v_h \rangle_K = 0,  \quad \forall v_h \in V_h   
%\end{multline}
%%\textit{2. Deterministic modes: for $j= 1,\ldots,R$, find $\tilde{U}^{n+1}_j \in V_h$ s.t.}
%\begin{multline} \label{eqn:numexp2-detmodes}
%\lrX{\frac{\tilde{U}^{n+1}_j - U^n_j}{\triangle t},v_h} +  
%	\lrX{\varepsilon \nabla \tilde{U}^{n+1}_j, \nabla v_h} 
%	+\lrX{\bar{\bu} \cdot \nabla \tilde{U}^{n+1}_j, v_h} 
%	+\lrX{ \mathbb{E}[{\bu}^{\star} \cdot \nabla u^{n} Y^n_j], v_h} 
%	\\ 
%	+ \sum_{K \in \Th} \frac{\delta_K}{\dt}\langle\tilde{U}^{n+1}_j - U^n_j, \bar{\bu} \cdot \nabla v_h\rangle_K 
%	+ \langle  \bar{\bu} \cdot \nabla \tilde{U}^{n+1}_j  + \mathbb{E}[ \bu^{\star} \cdot \nabla \uhr[n] Y^n_j ], \bar{\bu} \cdot \nabla v_h \rangle_K = 0,  \quad \forall v_h \in V_h  
%\end{multline}
%%\textit{3. Stochastic modes: find $\tilde{Y}^{n+1} \in \mathbb{R}^{N_C \times R}$ s.t.}
%\begin{multline}
%	(\tilde{Y}^{n+1} - Y^n) (\frac{\tilde{W}}{\dt} +  \lrX{\varepsilon \nabla (\tilde{U}^{n+1})^{\top}, \nabla \tilde{U}^{n+1}} + \lrX{(\bar{\bu} \cdot \nabla \tilde{U}^{n+1})^{\top}, \tilde{U}^{n+1} } 
%	+ \sum_{K \in \Th} \delta_K \langle (\bar{\bu} \cdot \nabla \tilde{U}^{n+1})^{\top}  ,  \bar{\bu} \cdot \nabla \tilde{U}^{n+1}  \rangle_K )
%	\\ + \mathcal{P}_{\mathcal{Y}}^{\perp} \lrX{\bu^{\star} \cdot \nabla u^{n}, \tilde{U}^{n,n+1}} 
%+ \sum_{K \in \Th} \delta_K \mathcal{P}_{\mathcal{Y}}^{\perp} \langle \bu^{\star}i \nabla u^{n}, \bu \cdot \nabla \tilde{U}^{n+1}\rangle_K
%	= \mathbf{0} 
%	\\\mathrm{in } \quad \Lthm. \label{eqn:bdet-stochmodes}
%\end{multline}
%
 
We repeat the same experiment under the same conditions as in the previous section; the plots for the total variation and variance are found in~\ref{fig:numexp2-tv} and~\ref{fig:numexp2-vars}

\begin{figure}[h]
\includegraphics[width=9cm]{stochb-vars-comparison}
\centering
\caption{Variance of the indiviual modes. 
}
\label{fig:numexp2-vars}
\end{figure}

In this setting, it is more apparent how the oscillations appearing in $U_0$ eventually contaminate $U_1$, and how the SUPG is successfull at mitigating those oscillations.  

\begin{figure}[h]
\includegraphics[width=9cm]{stochb-tv-comparison}
\centering
\caption{Total variation of the indiviual modes. 
}
\label{fig:numexp2-tv}
\end{figure}

Finally, we display a realisation of the DLR solution at $t = 2\pi$, again comparing the Galerkin and the SUPG-stabilised versions: 

\begin{figure}[h]
\includegraphics[width=15cm]{stochb-vn-real-2-3d}
\centering
\caption{A realisation of the numerical DLR solution obtained through Galerkin (left) and through the SUPG-stabilised method (right).} 
%The same color scheme is applied to both plots.}
\label{fig:stochb-real-dlr-vs-gal}
\end{figure}






==> sdraft/numexp3.tex <==
On the physical domain $D = (0,1)^2$ and on the time interval $[0,T]$ with $T=1$, we solve the transient random advection-diffusion-reaction~\eqref{eqn:adv-diff-reac}, with coefficients
\begin{align*}
	\varepsilon = 10^{-8}, && \bu = (1, -1)^{\intercal}, && c(\mathbf{y}) = 0.1 + y_1,
\end{align*}
with homogenous boundary conditions, and where $\mathbf{y} \in \Gamma = [0,1]^2$. The initial condition is given by $u_0(\mathbf{x}, \mathbf{y}) = \exp(- 10 y_2) \cdot d(\mathbf{x}, \mathbf{y})$, where 
\begin{equation*}
	d(\mathbf{x}, \mathbf{y}) = \left\{
		\begin{aligned}
			& 1  \text{ if } (x - x_0)^2 + (y - y_0) \leq 1 \text{ for } (x_0, y_0) = \left(0.25 + \frac{\cos(2\pi y_1)}{50}, 0.5 + \frac{\sin(2 \pi y_2)}{50} \right) \\
			& 0 \text{ else,}
		\end{aligned}
		\right.
\end{equation*}
corresponding to a family of cylinders with random heights and with origins slightly perturbed from $(0.25, 0.5)$. 

The solution obtained via the standard DLR method is compared to the SUPG-DLR method. Upon subtracting the mean from the field, 
we perform a (generalised) SVD and take the resulting $7$ first dominant modes as the initial condition (hence $R = 7$).  
%The realisations of the initial conditions are obtained from a cylinder of unit height and smoothed with a parameter depending on $\omega$. More precisely, $\displaystyle~u_0(x,\omega) = \mathcal{S}_{\omega}(v_0)$, where $v_0(\mathbf{x}) = 1$ if $(x - 0.25)^2 + (y - 0.75)^2 \leq 0.15^2$ and $0$ else, and $\mathcal{S}_{\omega}(v)$ is the solution operator to the problem $\displaystyle u - 10^{-4}\omega \Delta u = v$. This can be understood as one finite-difference-in-time step of a heat equation $\displaystyle \dot{u} - \omega \Delta u = 0$ with initial condition $u_0 = v$ and $\dt = 10^{-4}$. 
The discretised stochastic space is obtained by drawing $N_C = 1000$ uniformly distributed samples from $\Gamma$. The physical space is given by $\mathbb{P}^C_1(\mathcal{T}_h) = V_h \subset V$, where $\mathcal{T}_h$ is a non-periodic quasi-uniform triangulation of $D$ with dimension $N_h = \mathrm{dim}(V_h) = 6477$.   
%The full-order model discrete initial condition are obtained by computing $\mathcal{S}^h_{\omega_i}(v_{0})$, where $\mathcal{S}^h_{\omega_i}$ the solution operator to the same problem as $\mathcal{S}_{\omega_i}$ but in finite dimensions. The $R$-rank initial condition is obtained by taking a (TODO : weighted) singular values decomposition of the resulting matrix. 
%TODO: small issue with initial condition when \omega = 0...
%TODO : weighting parameter delta_K
Following the discussion in~\cite{jovo11}, for each cell $K \in \mathcal{T}_h$ we define $h_K = \nicefrac{\mathrm{diam}(K)}{\sqrt{2}}$ and set $\delta_K = \nicefrac{h_K}{4}$. We reiterate that, while it does not correspond to the scaling under which it is possible to prove stability of the method, it is well-known numerically that the scaling $\delta_K \propto h_K$ produces good numerical results for time-dependent problems. 

Finally, two metrics are used to quantify the oscillations. The first is given by the \textit{Maximal Difference} (called \textit{variance} in~\cite{josc08, jovo11}),
%\[
%	\mathrm{var}(u_{\hhmu}(t)) = \max_{(x, \omega) \in (D,\hat{\Omega})} u_{\hhmu}(t, x, \omega) - \min_{(x, \omega) \in (D,\hat{\Omega})} u_{\hhmu}(t, x, \omega)
%\]
and as our focus is on the stabilisation of the physical modes, we apply the Maximal Difference metric to each individual physical mode, i.e., 
\begin{equation} \label{eqn:variance-modes}
	\mathrm{MD}(U_i(t)) \coloneqq \max_{x \in D} U_i(x, t) - \min_{x \in D} U_i(x, t)
\end{equation}
A second measure of the oscillations is given by the total variation of each physical mode, given by the formula
\begin{equation} \label{eqn:tv-modes}
	\mathrm{TV}(U_i(t)) \coloneqq \int_{D} \| \nabla U_i(t)\|.
\end{equation}

The modal decomposition makes interpretability of the physical modes not straightforward. 
Nevertheless, neglecting the diffusion and advection term, the equation $\dot{u}+  c(\omega) u = 0$ displays pointwise exponential decay at rate $c(\omega)$. This decay must be reflected in the physical modes, as the stochastic ones are kept orthonormal. 
The variance metric can be used as a proxy to track this behaviour. The decay being more or less uniform, it thus corresponds to a general decay in amplitude; hence, the total variation norm is also expected to display the same type of decay. 
%Here we inspect the evolution of the oscillations at the level of the physical modes, where the oscillations are expected to arise in practice. Due to the reaction term, the predicted behaviour is an exponential decrease of the amplitude of the realisations; this can also be seen to hold true for the individual physical modes -- as evidenced by the decreasing trends in Figure~\ref{fig:vn4-vars-tv}, both metrics acting as a proxy for quantifying the amplitude of the function. 
For both plots in~Figure~\ref{fig:vn4-vars-tv}, the full lines indicate SUPG modes, while the dotted lines indicate standard Galerkin modes. The variances of the modes can be seen to be less oscillatory when using the SUPG method, indicating fewer oscillations with smaller amplitudes. The total variation metric also indicates that the SUPG modes display fewer oscillations; by nature, this metric is particularly sensitive to sharp oscillations, and as can be seen, the total variation of the SUPG modes decreases at a faster rate than that of the Galerkin modes.  



\begin{figure}[h]
\centering
\includegraphics[width=.5\textwidth]{tv-modes}%
\includegraphics[width=.5\textwidth]{vars-modes}
\caption{Total variation (left) and Maximal Difference (right) to quantify the oscillations of the physical modes $\{U_i\}_{i=0}^7$.
In all cases, the SUPG-stabilised modes read lower values than the corresponding standard Galerkin modes. 
%The maximal differences of SUPG-DLR modes appear more stable behaviour (clearer exponential decay, fewer oscillations, etc).
In the TV plot, the standard DLR modes decay significantly slower than the SUPG ones.
This indicates that many oscillations are present in all modes, unlike in the SUPG-DLR modes.   
}
\label{fig:vn4-vars-tv}
\end{figure}

% lower is better
% two metrics are to quantify the osillations
% neglecting the advection term

% can I write a justified argument ? correct norm-energy behaviour seems to be exponential decay - but those are L2 norms, but I have ``weird'' metrics ? 
% should have the same swaps, or none...
% the colors are a bit off, 


==> sdraft/old-f-bounds.tex <==
	\begin{align}
		|(f, \uhr[n+1]) + & \sum_{K \in \Th} \delta_K (f, \bu \cdot \nabla \uhr[n+1] )_{K,\Lthm}| \nonumber
		\\
																								&	\leq \|\mu_0^{-\nicefrac{1}{2}} f\|\|\mu_0^{\nicefrac{1}{2}} \uhr[n+1]\| + \sum_{K \in \Th} \delta_K \frac{\|\bu\| C_I}{h_K} \| \mu_0^{-\nicefrac{1}{2}} f \|_{K,\Lthm} \| \mu_0^{\nicefrac{1}{2}} \uhr[n+1]  \|_{K,\Lthm} \nonumber
		\\
																								&		\leq \|\mu_0^{-\nicefrac{1}{2}} f\|\|\mu_0^{\nicefrac{1}{2}} \uhr[n+1]\| +  \frac{1}{4C_I C_E^2}  \sum_{K \in \Th} \| \mu_0^{-\nicefrac{1}{2}} f \|_{K,\Lthm} \| \mu_0^{\nicefrac{1}{2}} \uhr[n+1]  \|_{K,\Lthm} \nonumber
		\\
																								&		\leq \frac{2}{\mu_0} \left(1 + \frac{1}{16 C_I^2 C_E^4}\right) \|f\|^2_{X,\Lthm} 
		+  \frac{1}{4}\| \mu^{\nicefrac{1}{2}} \uhr[n+1]\|^2_{X\Lthm}.
	\end{align}
However, if $\mu_0 = 0$, then we bound
	\begin{align}
		|(f, \uhr[n+1]) + & \sum_{K \in \Th} \delta_K  (f, \bu \cdot \nabla \uhr[n+1] )_{K,\Lthm}| \nonumber
		\\
																								&	\leq \|f\|\| \uhr[n+1]\| + \sum_{K \in \Th} \delta_K \frac{\|\bu\| C_I}{h_K} \| f \|_{K,\Lthm} \|\uhr[n+1]  \|_{K,\Lthm} \nonumber
		\\
																								&		\leq \|f\|\|\uhr[n+1]\| +  \frac{1}{4C_I C_E^2}  \sum_{K \in \Th} \| f \|_{K,\Lthm} \|\uhr[n+1]  \|_{K,\Lthm} 
		\\
																								&		\leq 
		\left(
			\frac{1}{2} + \frac{1}{8 C_I C_E^2}
		\right)
		\left(
			\|f\|^2_{X,\Lthm} + \|\uhr[n+1]\|^2_{X,\Lthm}
		\right).
	\end{align}



==> sdraft/scrap.tex <==
%and deriving evolution equations for the factors $U_i(t,x)$ and $Y_i(t, \omega)$. 
%it consists in seeking a low-rank approximation $Y(t) = U(t) S(t) V(t)^{\top}$ of $A$ of the type $\dot{A}(t) = F(t, A)$, with $A(t) \in \mathbb{R}^{m \times n}$. This is achieved by imposing that $Y$ verifies
%\begin{equation} \label{eqn:dlr-lubich}
%	\dot{Y}(t) \in \mathcal{T}_{Y(t)} \mathcal{M}_R \quad\mathrm{s.t.}\quad \| \dot{Y}(t) - F(Y(t))\| = \min,  
%\end{equation}
%where $\mathcal{M}_R \subset \mathbb{R}^{m \times n}$ is the differential manifold of rank-$R$ functions, and $\mathcal{T}_{Y(t)} \mathcal{M}_R$ the tangent space at $Y(t)$. Denoting by $P_{Y(t)}$ the orthogonal projection on the tangent space $\mathcal{T}_{Y(t)} \mathcal{M}_R$,~\eqref{eqn:dlr-lubich} can equivalently be rewritten as the following Galerkin condition on $\mathcal{M}_R$, 
%\begin{equation*}
%\dot{Y}(t) = P_{Y(t)} F(Y(t)),
%\end{equation*} 
%and thus the DLR framework can be understood as (\textit{orthogonally}) projecting the dynamics on the tangent space at $Y(t)$. 

%This framework relies on on-the-fly update of the bases $U(t)$ and $V(t)$ on which the dynamics are projected, and marks its difference to other model order reduction techniques such as the Proper Orthogonal Decomposition which are based on an online/offline paradigm.  
%The modes $U(t) \in \mathbb{R}^{m \times R}$, $S(t) \in \mathbb{R}^{R \times R}$ and $V(t) \in \mathbb{R}^{n \times R}$ ($R$ hereafter denotes the \textit{rank}) are characterised by evolution equations; under some further assumptions, solving the factor equations is significantly cheaper than solving the full-order model, and thus computationally attractive. Many aspects of dynamical low rank systems have since then been investigated~\cite{luos14, kueice23, eijo21, eilu18, kiva19, cavama23}.
%TODO : make this sentence a bit better... ? 
%The connection to random PDEs should appear quite naturally when considering that random fields discretised both in physical and stochastic space are essentially matrices.

%In the context of random PDEs, this approach has been independently investigated in~\cite{sale09} under the name of Dynamically Orthogonal (DO) method with a seemingly different starting point.
%Given a random problem $\dot{u} + \mathcal{L}u = f$, the authors proposed to search for an approximation of the true random field by mimicking a truncated Karhunen-Loève expansion 
%\begin{equation} \label{eqn:do-exp}	
%	u_{\mathrm{true}}(t,x,\omega) \approx u_{\mathrm{DO}}(t,x,\omega) = \sum_{i=1}^R U_i(t,x) Y_i(t,\omega), 
%\end{equation}
%and deriving evolution equations for the factors $U_i(t,x)$ and $Y_i(t, \omega)$. 
%One subtle but key difference between these two setting is that, in the DO equations, the projections that arise are obtained using the scalar products of the original spaces, while in the standard DLR setting, the projections are obtained post-discretisation by using the standard $L^2$-product in $\mathbb{R}^n$. (More recently, the former approach has been introduced in the dynamical low rank community under the name ``continuous DLR''). 
%This ``loss of structure'' seems to lead to further instabilities as has been discussed in~\cite{kueice23} -- for this reason among others, 
%We now propose to ``build in'' the PG formalism within the DLR framework. We start by proposing a heuristic construction of the Petrov-Galerkin framework. The main idea is to mimic the original derivation of the DLR constitutive equations, which are based on a minimisation problem, namely
%
%
%\textit{Find $v \in \mathcal{T}_{\!\!u} \mathcal{M}_R$ s.t.}
%\[
%	v = \argmin_{w \in \TuMR} \|w + Lu\|. 
%\]
%(where the norm is induced by some suitable scalar product $(\cdot, \cdot)$). 
%We start from the same point, but this time take the norm to be induced by some scalar product induced by a symmetric, positive-definite operator $\Hcal$, i.e., $(u,v)_{\Hcal} = (u, \Hcal v) = (\Hcal u, v)$ and $\|u\|^2_{\Hcal} = (u,u)_{\Hcal}.$
%
%\textit{Find $v \in \TuMR$ s.t.}
%\[
%	v = \argmin_{w \in \TuMR} \|w + Lu\|_{\Hcal}. 
%\]
%%We furthermore assume that $\Hcal$ induces a bijection between $\TuMR$ and its image. 
%This condition is equivalent to fulfilling the following variational formulation,  
%\begin{equation}
%	(\partial_t u, v)_{\Hcal} + (Lu, v)_{\Hcal} = 0 \quad \quad \forall v \in \TuMR . 
%\end{equation}
%%Now, $u(t)$ belongs to some space $U$ and 
%%We define $\Pi_u$ to be the orthogonal projection onto $\TuMR$, defined by
%%
%%\[
%%	\Pi_u(v) = \argmin_{w \in \TuMR} \|w - u\|.
%%\]
%%Note that we are using the first norm. While it is possible to use the $\Hcal$-induced norm (in which the developed framework will be similar to the standard DLR framework with different scalar products), we refrain from doing so, anticipating when the operator $\Hcal$ will not be assumed to induce a norm. 
%%Using the definitions of the scalar product and the fact that $\partial_t u \in \TuMR$ to obtain the problem: 
%
%In light of the discussion in section~\ref{subsec:not}, we then propose to take the following problem as the basis of the DLR-PG framework:
%
%\noindent \textit{Find } $u: (0,T] \rightarrow V_h \otimes \Lthm$  \textit{ s.t.}
%\begin{equation} \label{eqn:PG-start}
%	(\dot{u}, \Hcal v_{\hhmu})_{X, \Lthm} + L_h(u , v_{\hhmu}) = 0, \qquad \forall v_{\hhmu} \in \TuMR, \mathrm{a.e.}\; t \in (0,T]
%\end{equation}
%
%%
%%\textit{Find } $\partial_t u \in \TuMR$ \textit{s.t.} 
%%\begin{equation} \label{eqn:PG-start}
%%(\partial_t u, \Pi_u \Hcal v) + (Lu, \Hcal v) = 0 \quad \forall v \in \TuMR
%%\end{equation}
%%% comment on what happens if using the induced by the energy norm
%% comment on U, V must belong to some bigger space
%We shall use~\eqref{eqn:PG-start} as a starting point, \textit{dropping the requirement that $\Hcal$ be symmetric positive-definite operator}. While this leads to the loss of interpretation of the problem as a minimisation problem, it nonetheless allows to establish a framework in which the dynamics are meaningfully constrained to the tangent space.   
%%TODO : what are the consequnces of that ??? what more is there to say???
%%In the case of SUPG, we choose $\Hcal = (I + \alpha \mathbf{b} \cdot \nabla)$; whether $\mathbf{b}$ is stochastic or not will significantly impact how hard (or easy) it is to solve this problem.  
%
%We introduce a fuller characterisation of $\TuMR$ in the discretised setting, discussing the choice of standart basis, ensuing mass matrix and consequences for the DLR framework (and SUPG).
%
%To fix ideas, we consider the random field on the tensor-product space $V_h \otimes L^2_{\hat{\rho}}$, where $V_h = \mathbb{P}^C_1(\Th)$. 
%At a point $u = \sum_{i=1}^R U_i Y_i $, we consider the basis given by 
%\begin{align*}
%	\{ \phi_i Y_j  \} = \{e_{ij}\} && i = 1, \ldots, \mathrm{d.o.f}, \quad j = 1, \ldots, R \\
%	\{ U_i z^j  \} = \{ f_{ij} \} && i = 1, \ldots, R,\quad j = 1, \ldots, N_C - R,
%\end{align*}
%where $\psi^j$ is an orthonormal basis of $\mathcal{Y}^{\perp}$, and $\{\phi_i\}$ is a basis of $V_h$. The following relations prove crucial for uncoupling the DLR equations: 
%\begin{align*}
%	(e_{ij}, e_{kl}) = \delta_{jl} \cdot (\phi_i, \phi_k)_H && (e_{ij}, f_{kl}) = 0 && (f_{ij}, f_{kl}) = \delta_{jl}  \cdot (U_i, U_k)_H
%\end{align*}
%We now order the basis elements such that ``free'' part of the basis evolves the quickest ($[e_{11}, e_{21}, \ldots, e_{12}, \ldots, f_{11}, f_{12}, \ldots]$). Finally, we denote $M$ the mass matrix $M_{ij} = (\phi_i, \phi_j)_H$ and $\tilde{M}$ the mass matrix of the $U$-basis, i.e.,  $\tilde{M}_{ij} = (U_i, U_j)_H$. 
%The mass matrix is then given by 
%\begin{equation*}
%	\mathbf{M} =
%	\begin{bmatrix}
%		I_R \otimes M & \mathbf{0} \\
%		\mathbf{0} & \tilde{M} \otimes I_{N_C - R}
%	\end{bmatrix}
%\end{equation*}
%This structure proves to be crucial when solving the DLR equations, as it allows to uncouple the system and solve $R$ systems of size $\mathrm{d.o.f}$ and a (coupled) system of $R$ equations of size $N_C - R$ -- note that in practice, there is no need to keep track of the explicit values of the stochastic orthonormal basis $\mathcal{Y}^{\perp}$, and the system is solved on $L^2_{\hat{\rho}}$  and constrained to $\mathcal{Y}^{\perp}$. The inverse of this matrix is also block-diagonal, given by (using standart properties of the Kronecker product)
%\begin{equation*}
%	\mathbf{M}^{-1} =
%	\begin{bmatrix}
%		I_R \otimes M^{-1} & \mathbf{0} \\
%		\mathbf{0} & \tilde{M}^{-1} \otimes I_{N_C - R}
%	\end{bmatrix}
%\end{equation*}
%The upper left part can be put in relation to projecting the projection of $v$ on $V_h$ on $\mathrm{span} \mathcal{Y}$, whereas the lower-right part corresponds to projecting the projection of $v$ on $\mathrm{span}\, U$ on $\mathcal{Y}^{\perp}$.
%
%We point out that there is a strong correspondence between deriving evolution equations by ``testing'' against the correct test functions and Lubich's projector-splitting equations. Firstly, the DO equations and the continuous DLR equations are in essence the same (Lubich goes through the Galerkin projection, Lermusiaux uses the strong form, but same idea); the projector-splitting has been shown to be the same to Eva's algorithm \textit{if the dynamics are approximated by a quadrature}. The splitting of the projector (i.e., solving each sub-problem part-by-part) can also be obtained by testing against the adequate test functions. Note that this would in theory require choosing a set of test functions that evolve in time, but we follow Eva's approach and will subsequently ``freeze'' the stochastic (resp. phyiscal) basis. In short: if we can find test functions that decouple (or are orthogonal to a part of the derivative), this can be interpreted as a splitting with hopefully interesting properties.  
%
%\underline{Case I : $\mathbf{b}$ deterministic, $\varepsilon$ stochastic}
%We consider the same operator 
%\[
%	Lu = -\varepsilon \Delta u + \mathbf{b} \cdot \nabla u
%\]
%where the diffusion $\varepsilon$ is assumed to be stochastic, while $\mathbf{b}$ is deterministic. In that case, $\Hcal = I + \alpha \mathbf{b} \cdot \nabla$ only changes the physical test space -- crucially, it doesn't alter the tensor-product structure of the test space or the orthonormality of the stochastic basis. We therefore choose the test functions $\tilde{e}_{ij} = \Hcal e_{ij} = (\phi_i + \alpha \mathbf{b} \cdot \nabla \phi_i) Y_j$ and $\tilde{f}_{ij} = \Hcal f_{ij} = (U_i + \alpha \mathbf{b} \cdot \nabla U_i) \psi_j$. 
%We enforce the constraint on the boundary condition by imposing that $\partial_t u = \sum_{i=1}^R \dot{U}_i Y_i + U_i \dot{Y}_i$, with the usual gauge condition $\mathbb{E}[\dot{Y}_i Y_j] = 0$. 
%Testing~\eqref{eqn:PG-start} against $\tilde{e}_{ij}$, we obtain
%\[
%	(\dot{U}_j, \phi_i + \alpha \mathbf{b} \cdot \nabla \phi_i)_H + (Lu Y_j , \phi_i + \alpha \mathbf{b} \cdot \nabla \phi_i)_{H, L^2_{\rho}} = 0 \quad \forall i = 1,\ldots,\mathrm{d.o.f.}
%\]
%Rewriting, we obtain
%\begin{equation} \label{eqn:detb-detmodes}
%	(\dot{U}_j,v_h + \alpha \mathbf{b} \cdot \nabla v_h)_H + (\mathbb{E}[Lu \, Y_j], v_h)_{V^{\prime}V, L^2_{\hat{\rho}}} + \alpha (\mathbf{b} \cdot \nabla u, \mathbf{b} \cdot \nabla v_h ) = 0, \quad \forall v_h \in V_h 
%\end{equation}
%Applying the same technique with $\tilde{f}_{ij}$, we obtain
%\begin{multline*}
%	\sum_{i=1}^R (\dot{Y}_i, \psi_j )_{L^2_{\hat{\rho}}}(U_i, U_j + \alpha \mathbf{b} \cdot \nabla U_j)_{H} + (Lu , (U_j + \alpha\mathbf{b} \cdot \nabla U_j)\psi_j)_{H, L^2_{\rho}} = 0 
%	\\ \forall 1 \leq i \leq R, 1 \leq j \leq N_C - R
%\end{multline*}
%This may also be rewritten 
%\begin{equation} \label{eqn:detb-stochmodes}
%	\dot{Y} W + \mathcal{P}_{\mathcal{Y}}^{\perp}[(Lu, U + \alpha \mathbf{b} \nabla U)_{V^{\prime},V}] = \mathbf{0} \quad \mathrm{in } \quad L^2_{\hat{\rho}}, 
%\end{equation}
%where $Y = (Y_1, \ldots, Y_R)$, $U = (U_1, \ldots, U_R)$ and $W_{ij} = (U_i, U_j + \alpha \mathbf{b} \nabla U_j)$. 
%
%From there, we can discretise in time by applying a projector-splitting strategy similar to the one used by Eva; the equations therefore become
%\begin{gather} \label{eqn:bdet-allmodes}
%	(\frac{U^{n+1}_0 - U^n_0}{\triangle t},v_h + \alpha \mathbf{b} \cdot \nabla v_h)_H +  (\mathbb{E}[- \varepsilon \Delta u^{n,n+1} + \bu \cdot \nabla u^{n,n+1}], v_h + \alpha \bu \cdot \nabla v_h)_{V^{\prime}V, L^2_{\hat{\rho}}} 
%	%+ \alpha (\mathbf{b} \cdot \nabla u^{n,n+1}, \mathbf{b} \cdot \nabla v_h ) 
%	= 0, \quad \forall v_h \in V_h \\  
%	(\frac{\tilde{U}^{n+1}_j - U^n_j}{\triangle t},v_h + \alpha \mathbf{b} \cdot \nabla v_h)_H 
%	+ (\mathbb{E}[(- \varepsilon \Delta u^{n,n+1} + \bu \cdot \nabla u^{n,n+1})Y^n_j], v_h + \alpha \bu \cdot \nabla v_h)_{V^{\prime}V, L^2_{\hat{\rho}}} 
%	%+(\mathbb{E}[- \varepsilon \Delta u^{n,n+1} \, Y_j], v_h)_{V^{\prime}V, L^2_{\hat{\rho}}} + \alpha (\mathbf{b} \cdot \nabla u^{n,n+1}, \mathbf{b} \cdot \nabla v_h ) = 0, \quad \forall v_h \in V_h 
%	\label{eqn:bdet-detmodes} \\ 
%	\frac{\tilde{Y}^{n+1} - Y^n}{\triangle t} \tilde{W} + \mathcal{P}_{\mathcal{Y}}^{\perp}[(- \varepsilon^{*} \Delta u^{n,n+1} + \bu \cdot \nabla u^{n,n+1}, \tilde{U}^{n+1} + \alpha \mathbf{b} \nabla \tilde{U}^{n+1})_{V^{\prime},V}] = \mathbf{0} \quad \mathrm{in } \quad L^2_{\hat{\rho}}, \label{eqn:bdet-stochmodes}
%\end{gather}
%where $\tilde{W}_{ij} = (\tilde{U}^{n+1}_i, \tilde{U}^{n+1}_j + \alpha \mathbf{b} \cdot \nabla \tilde{U}^{n+1}_j)_H$
%
%This stabilisation approach could also be used for a stochastic transport term with moderate stochasticity.
%
%
%\underline{Case II : $\mathbf{b}$ stochastic $\varepsilon$ deterministic}
%We consider the same operator 
%\[
%	Lu = -\varepsilon \Delta u + \mathbf{b} \cdot \nabla u
%\]
%This case is much more difficult, as the orthogonality relation between the image space and original space in the stochastic modes is now lost.
%We recall that for $v \in \TuMR$, $w = \Hcal v$, we have
%\begin{multline*}
%	\Pi_u[\Hcal v] = \Pi_u[v + \alpha \mathbf{b} \cdot \nabla v] = v + \alpha \Pi_u [\mathbf{b} \cdot \nabla v] \\ = v + \alpha \mathcal{P}_{\mathcal{Y}}[\mathcal{P}_{V_h}[\mathbf{b}\cdot \nabla v]] + \alpha \mathcal{P}_{\mathcal{Y}}^{\perp}[\mathcal{P}_{\mathcal{U}}[\mathbf{b} \cdot \nabla v]],
%\end{multline*}
%which ``skews'' the test space. Nevertheless, notice how the dominant part is $v$, which translates in a ``block-diagonal'' structure. Indeed, the mass matrix(basis vs. new basis) now has the following shape: 
%\[
%	\mathbf{N} = \mathbf{M} + \alpha \mathbf{B} 
%\]
%which suggests using a block-Jacobi iterative method, essentially allowing to solve the system iteratively using the same decoupling+splitting strategy as before.
%Note: there are some simplifications on the $\mathbf{B}$ matrix, but nothing substantial. 
%
%TODO : evolving ``doubly orthogonal basis'': started looking into it, can't find clean equation that don't involve messy constructions. 
%
%\vspace{1em}
%
%\underline{Oblique/skewed projection interpration. }
%
%It is interesting to notice that the time-integration proposed above has an interpretation as a ``skewed'' projection.  
%as an oblique projection on $\mathcal{T}_{\!u}\mathcal{M}_{R}$ parallel to $\mathcal{S}_2$, where $\mathcal{S}_2^{\perp} = (I + \alpha \bu \cdot \nabla) V_h \otimes L^2_{\hat{\rho}}$. 
%For simplicity, we assume $\bu$ to be divergence-free and
%% PG projection for the physical modes + combine. 
% 
%Indeed, taking~\eqref{eqn:bdet-detmodes}, multiplying by $Y_i$ and summing we obtain
%\begin{multline*}
%	\sum_{j=1}^R	(\frac{\tilde{U}^{n+1}_j Y_j^n - U^n_j Y^n_j }{\triangle t},v_h + \alpha \mathbf{b} \cdot \nabla v_h)_H 
%	\\ 
%	+ (\mathcal{P}_{\mathcal{Y}}[- \varepsilon \Delta u^{n,n+1} + \bu \cdot \nabla u^{n,n+1}], v_h + \alpha \bu \cdot \nabla v_h)_{V^{\prime}V, L^2_{\hat{\rho}}} %+ \alpha (\mathcal{P}_{\mathcal{Y}}\mathbf{b} \cdot \nabla u^{n,n+1}, \mathbf{b} \cdot \nabla v_h ) 
%	= 0. 
%\end{multline*}
%Whereas by taking~\eqref{eqn:bdet-stochmodes} in their weak form, inverting the $\tilde{W}$, right-multiplying by $\tilde{U}^{n+1, \top}$, we obtain
%\begin{multline*}
%	\sum_{j=1}^R \frac{\tilde{U}^{n+1}_j \tilde{Y}^{n+1}_j - \tilde{U}_j^{n+1}Y^n_j}{\triangle t} + \mathcal{P}^{\perp}_{\mathcal{Y}}[\mathcal{P}_{\mathcal{U}, \mathcal{U} + \alpha \mathbf{b} \cdot \nabla \mathcal{U}}[- \varepsilon \Delta u^{n,n+1} + \bu \cdot \nabla u^{n,n+1}]]
%\end{multline*}
%The former equality also holds when taking the weak form in $L^2_{\hat{\rho}}$, and the latter holds when testing against $v_h + \alpha \bu \cdot \nabla v_h$; consequently, we have, summing these two equations, 
%\begin{multline*}
%	\langle \frac{u^{n+1} - u^{n}}{\triangle t}, (v_h + \alpha \cdot \bu \nabla v_h)z \rangle_{H,L^2_{\hat{\rho}}} 
%	\\ + (\tilde{\Pi}_u [-\varepsilon \Delta u^{n,n+1} + \bu \cdot \nabla u^{n,n+1}], (v_h + \alpha \cdot \bu \nabla v_h)z)_{V^{\prime}V,L^2_{\hat{\rho}}},
%\end{multline*}
%where $\tilde{\Pi}_u[v] = \mathcal{P}_{\mathcal{Y}}[v] + \mathcal{P}^{\perp}_{\mathcal{Y}}[\mathcal{P}_{\mathcal{U}, \mathcal{U} + \alpha \mathbf{b} \cdot \nabla \mathcal{U}}[v]]$, $v_h \in V_h$ and $z \in L^2_{\hat{\rho}}$, which would be more in line with the notion of generalised projector.  
%
%Note : also possible to ``pass'' $\Hcal$ to the other side? Feels like the test against $v_h + \alpha \cdot \bu \nabla v_h$ rather than $v_h$ is redundant... Need to check that everything works fine, would have to interpret the $U$-modes as the oblique projection of $\mathcal{P}_{V_h, \Hcal V_h}$ and would then have a modified projector $\hat{\Pi} = \mathcal{P}_{V_h, \Hcal V_h} \mathcal{P}_{\mathcal{Y}} + \mathcal{P}_{\mathcal{Y}}^{\perp} \mathcal{P}_{\mathcal{U}, \mathcal{U} + \alpha \mathbf{b} \cdot \nabla \mathcal{U}}$. 
%
%% Tangent space interpretation + tangent space formulation
%
%TODO: work out the properties of the projector $\tilde{\Pi}_u$ + implications. 
%
%TODO: need to verify implications that $\alpha \bu \cdot \nabla$ disappears in stochastic equation -- should play fine, as the term simply dies out and can be added. 
%
%
%\vspace{1em}
%
%\underline{Generalisation of the projection-on-tangent-space-operator}
%
%TO WRITE DOWN. 
%
%\vspace{1em}
%
Following the steps of the proof of~\cite{sale09}, the first set of equations of~\eqref{eqn:dlr-weak-form} are obtained by testing against $v_{\hhmu} = v_h Y_j \in \TuMRa[,\hmu]$ for $j = 0,\ldots,R$. 
Indeed, the first term $(\dot{u}, v_{\hhmu})$, as $\dot{u} = \dot{U}_0 Y_0 + \sum_{i=1}^R \dot{U}_i Y_i + U_i \dot{Y}_i$, verifies
%TODO: find sources for the well-posedness of time-dependent problems in Petrov-Galerkin framework.  
%Indeed, the tangent space $\TuMR = \{ \sum_{i=0}^R \delta v_i Y_i + U_i \delta z_i \;\text{s.t.}\; \langle Y_i, Y_j \rangle_{\hat{\mu}} = \delta_{ij},   \langle Y_i, \delta z_j \rangle_{\hat{\mu}} = 0 \}$. We seek to obtain evolution equations of the terms $\dot{U}_i$ and $\dot{Y}_i$ for $i = 1, \ldots, R$, as they constitute $\partial_t u = \sum_{i=1}^R \dot{U}_i Y_i + U_i \dot{Y}_i$. Analogously to what was done in~\cite{kolu07}, the evolution equations for the physical modes are obtained by testing against suitable test functions. Testing $\delta v Y_j$ against $\partial_t u$, we obtain
\begin{align*}
	(\dot{u}, v_h Y_j )_{X,\Lthm} &= \sum_{i=0}^R(\dot{U}_i Y_i + U_i \dot{Y}_i, v_h Y_j)_{X,\Lthm} =
	\\ &= \sum_{i=0}^R \langle \dot{U}_i, v_h  \rangle_X \langle Y_i, Y_j \rangle_{\hmu} + \langle U_i, v_h  \rangle_X \langle \dot{Y}_i, Y_j \rangle_{\hmu}
	\\ &= \langle \dot{U}_j,  v_h \rangle_X,  
\end{align*}
where both properties were used.  
%in the second line we made use of the tensor-product nature of the scalar product $(\cdot, \cdot)_{X,\Lthm}$ and in the third line, we used the parametrisations of the stochastic modes and the tangent space. 
Thus, also replacing $v_{\hhmu} = v_h Y_j$ in the remaining terms of~\eqref{eqn:PG-start} allows to derive an evolution equation of the form $\langle \dot{U}_i, v_h  \rangle_X + \texttt{rhs} = 0$. 

An analogous expression can be obtained for the stochastic modes by testing against $U_j z$ (for $z$ in $\mathcal{Y}^{\perp} \subset L^2_{\hmu,0}(\hat{\Omega})$) 
\begin{align*}
	(\dot{u}, U_j z )_{X,\Lthm} 
	= \sum_{i=0}^R \langle \dot{U}_i, U_j  \rangle_X \langle Y_i, z \rangle_{\hmu} + \langle U_i, U_j  \rangle_X \langle \dot{Y}_i, z \rangle_{\hmu}
	= \sum_{i=1}^R M_{ij} \langle \dot{Y}_i, z \rangle,
\end{align*}
where the tensor-product nature of the scalar product and the orthogonality relationships were yet again used. 
%as well as the fact that $\langle Y_i, z \rangle = 0$ for $1 \leq i \leq R$.  
The evolution coefficients are coupled through the Gram matrix $M_{ij} = \langle U_i, U_j \rangle_X$. 
%TODO: On a practical level, we expect the stabilisation to be mostly employed to deal with physical stabilisation.  
%TODO: idea for splitting operator
%TODO: generalising the idea to broader class of pbs

%The apparently more general class of problems where the mass matrix is given by
%\[
%	\tilde{\mathbf{M}} = 
%	\begin{bmatrix}
%		A \otimes B & C \otimes D \\
%		\mathbf{0} & E \otimes F
%	\end{bmatrix}
%\]
%is in fact non-realistic due to the arbitrariness of the stochastic basis.  

%We also introduce $(( u , v )) = $
%\todo{introduce new scalar product notation?}
%We consider an operator of the form $\Hcal = \Hcal_1 \otimes \Hcal_2$ be a separable operator such that either $\Hcal_1$ or $\Hcal_2$ induces a scalar product on the space on which it acts. Here, we will consider the case where this role is held by $\Hcal_2$ (operator acting on the stochastic space). 
%As $\Hcal_2$ acts on $\Lthm$ to itself (and $\Lthm$ is finite dimensional), it must be a bijection and $\Hcal_2^{-1}$ is well defined. For convenience, we will assume that $\Hcal_2$ enjoys uniform continuity and coercivity w.r.t $N_C$, i.e., 
%\begin{align*}
%	\mathbb{E}_{\hat{\mu}}[Y \Hcal_2 Y] \geq d \| Y  \|^2_{\Lthm}, 
%	&& 
%	\mathbb{E}_{\hat{\mu}}[Y \Hcal_2 Z] \leq D \| Y  \|_{\Lthm} \| Z\|_{\Lthm},
%	&&
%	\forall Y,Z \in \Lthm, \forall N_C \geq R,
%\end{align*}
%for some $D,d > 0$ indenpedent of $N_C$. This is not a necessary condition, and indeed for a fixed $N_C$, one may choose to define an \textit{ad hoc} operator $\Hcal_2$ verifying the necessary conditions. 
%In what follows, we use the following notation: 
%\begin{align*}
%	\langle Z, Y  \rangle_{\hat{\mu}} = \mathbb{E}_{\hat{\mu}}[Z Y] && \lrrt{Z,Y} = \mathbb{E}_{\hat{\mu}}[ Z \Hcal_2 Y] 
%	%\lrH{u,v} = \int_{\Omega} u v && \dpV{\mathcal{S},u} 
%\end{align*}
%%We introduce the following scalar products on $V_h \otimes L^2_{\hat{\mu}}(\hat{\Omega})$
%\begin{align*}
%	( uZ, vY )= \langle u,v \rangle_{X} \langle Z,Y \rangle_{\hat{\mu}} , &&
%	\dpr{uZ,vY} = \langle u, v \rangle_{X} \lrrt{Z,Y} , 
%\end{align*}


==> sdraft/si-norm-stab-old.tex <==
As the implicit Euler is an impractical algorithm for DLR schemes due to its very coupled nature, we are interested in using other time-integration schemes that to reach a balance between computability and desirable stability properties. One such choice is given by the semi-implicit time-stepping scheme. The desirable properties of this scheme become apparent under moderate stochasticity; we make the following assumtions: 
\begin{gather}
	\varepsilon^{\star}(\omega) \leq C_1 \varepsilon(\omega) \label{eqn:varepscond} \\
	|c^{\star}(x, \omega)| \leq \sqrt{1 - \delta} |c(x, \omega)| \label{eqn:cstarcond},
\end{gather}
and we furthermore assume that $\bu$ is divergence-free, i.e., $\nabla \cdot \bu = 0$. 

In what follows, we establish norm-stability bounds for the numerical solution under a hyperbolic CFL condition as well as a condition on $\delta_K$.

%TODO: likely something wrong with the max-mins
%TODO: is the Volker bound the same idea, but a slightly sharper bound of Gronwall type?
%TODO: remarks about the special case when div(b) = 0. 

\begin{theorem}
	For a general advection-diffusion-reaction operator such that TODO, TODO and TODO hold; then, for
	\begin{equation} \label{eqn:deltaK-si-cond}
		\delta_K \leq \cdots
	\end{equation}
	the iterates $\{\uhr[k]\}_{k=0}^N$ satisfy
	\begin{equation} \label{eqn:si-bound}
		a \leq b
	\end{equation}
\end{theorem}
\begin{proof}
	We test~\eqref{eqn:varf-adr-disc-si} against $\uhr[n+1]$. 
	The first term is developped as usual, 
	\[
		\frac{1}{2\dt}(\|\uhr[n+1] \|_{X,\Lthm}^2 -  \| \uhr[n] \|_{X,\Lthm}^2 +  \| \uhr[n+1]- \uhr[n] \|_{X,\Lthm}^2). 
	\]
	We then add and subtract the quantity
	\begin{equation}
		(\varepsilon^{\star} \nabla \uhr[n+1], \nabla v_{\hhmu}) + (c^{\star} \uhr[n+1], v_{\hhmu}) + \sum_{K \in \Th} (- \varepsilon^{\star} \Delta \uhr[n+1] + c^{\star} \uhr[n+1], \bu \cdot \nabla v_{\hhmu})_K, 
	\end{equation}
	allowing us to recover the variational formulation of the implicit Euler with some extra terms: 
	\begin{multline*}
		\frac{1}{2\dt}(\|\uhr[n+1] \|_{X,\Lthm}^2 -  \| \uhr[n] \|_{X,\Lthm}^2 +  \| \uhr[n+1]- \uhr[n] \|_{X,\Lthm}^2) + \aSUPG(\uhr[n+1], \uhr[n+1])
		\\ 
		+ \sum_{K \in \Th} \frac{\delta_K}{\dt} (\uhr[n+1] - \uhr[n], \bu \cdot \nabla \uhr[n+1]) = (f, \uhr[n+1]) + \sum_{K \in \Th} \delta_K (f, \bu \cdot \nabla \uhr[n+1]) 
		\\ + (\varepsilon^{\star} \nabla (\uhr[n+1] - \uhr[n]), \nabla \uhr[n+1]) + (c^{\star} (\uhr[n+1] - \uhr[n]), \uhr[n+1]) 
		\\ 
		+ \sum_{K \in \Th} \delta_K (- \varepsilon^{\star} \Delta(\uhr[n+1] - \uhr[n]) + c^{\star} (\uhr[n+1] - \uhr[n]), \bu \cdot \nabla \uhr[n+1])_K
	\end{multline*}
	We then bound the following terms: 
	\begin{align}
		|(\varepsilon^{\star} \nabla (\uhr[n+1] - \uhr[n]), \nabla \uhr[n+1])| &\leq \frac{C_I^2}{2 h^2} \|\uhr[n+1] - \uhr[n]\|_{X,\Lthm}^2 + \frac{C_1 }{2} \| \varepsilon\nabla \uhr[n+1]\|^2_{X, \Lthm}
		\\
		|(c^{\star} (\uhr[n+1] - \uhr[n]), \uhr[n+1])| &\leq \frac{1}{2}\|\uhr[n+1] - \uhr[n]\|_{X,\Lthm}^2 +\frac{1}{2}\|c^{\star} \uhr[n+1] \|^2_{X, \Lthm}  \\
		|(- \varepsilon^{\star} \Delta (\uhr[n+1]- \uhr[n]), \bu \cdot \nabla \uhr[n+1])_K| &\leq \trnorm{\varepsilon^{\star}}_K \frac{C_I^4}{h^4} \|\uhr[n+1] - \uhr[n]\|^2_{K,\Lthm} + \|\bu \cdot \nabla \uhr[n+1]\|^2_{K,\Lthm}
		\\
		|(c^{\star} (\uhr[n+1] - \uhr[n]), \bu \cdot \nabla \uhr[n+1])_K| &\leq \frac{1}{2} \trnorm{c^{\star}}_K \|\uhr[n+1] - \uhr[n]\|_{K,\Lthm}^2 +\frac{1}{2}\|\bu \cdot \nabla  \uhr[n+1] \|^2_{K, \Lthm} 
	\end{align}
	Furthermore, we have that
	\begin{gather}
		|(f, \uhr[n+1])| \leq \| \mu^{-1/2} f\|_{X,\Lthm} \|\mu^{1/2}\uhr[n+1] \|_{X,\Lthm} \leq \frac{1}{2\mu_0} \|f\|^2_{X, \Lthm} + \frac{1}{2}\| \mu^{1/2} \uhr[n+1] \|^2_{X, \Lthm} 
		\\
		\delta_K |(f, \bu \cdot \nabla \uhr[n+1])_K| \leq \frac{\delta_K}{2} \|f\|^2_{K,\Lthm} + \frac{\delta_K}{2} \| \bu \cdot \nabla \uhr[n+1] \|^2_{K,\Lthm}
	\end{gather}

\end{proof}
%TODO: the first line, something fishy...
%TODO: need to change the trnorm notation
%TODO: also the _K notation. 

